Raise a Child in Large Language Model: Towards Effective and Generalizable Fine-tuning

Recent pretrained language models extend from millions to billions of parameters. Thus the need to fine-tune an extremely large pretrained model with a limited training corpus arises in various downstream tasks. In this paper, we propose a straightforward yet effective fine-tuning technique, Child-Tuning, which updates a subset of parameters (called child network) of large pretrained models via strategically masking out the gradients of the non-child network during the backward process. Experiments on various downstream tasks in GLUE benchmark show that Child-Tuning consistently outperforms the vanilla fine-tuning by 1.5~8.6 average score among four different pretrained models, and surpasses the prior fine-tuning techniques by 0.6~1.3 points. Furthermore, empirical results on domain transfer and task transfer show that Child-Tuning can obtain better generalization performance by large margins.

==> float/table-nli-mnli.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
    \begin{tabular}{lccccc}
    \toprule
    & \bf Vanilla & \bf CF & \Delta & \bf CD & \Delta \\
    \midrule
    MNLI & 75.30 & 75.95 & 0.65 & 76.61 & 1.31 \\
    MNLI-M & 76.50 & 77.79 &  1.29 & 77.98 & 1.48 \\
    SNLI & 69.61 & 70.35 & 0.74 & 71.17 & 1.56 \\
    SICK & 48.25 & 49.13 & 0.88 & 50.15 & 1.90 \\
    SciTail & 73.65 & 75.42 & 1.77 & 75.08 & 1.43 \\
    QQP & 71.37 & 72.24 & 0.87 & 72.67 & 1.30 \\
    \midrule
    Mean & 69.11 & 70.15 & 1.04 & 70.61 & 1.50 \\
    \bottomrule
    \end{tabular}
}
\caption{The models are trained on MNLI with different fine-tuning methods and test on out-of-domain data directly.
CF: Child-tuning-F. CD: Child-tuning-D.
}
\label{table:nli-mnli}
\end{table}


==> float/table-nli-snli.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
    \begin{tabular}{lccccc}
    \toprule
    & \bf Vanilla & CF & \Delta & \bf CD & \Delta \\
    \midrule
    MNLI & 65.80 & 66.01 & 0.21 & 66.82 & 1.02 \\
    MNLI-M & 67.71 & 67.27 & -0.44 & 68.48 & 0.77 \\
    SNLI & 82.90 & 83.17 & 0.27 & 83.66 &  0.76 \\
    SICK & 51.50 & 51.16 & -0.34 & 51.42 & -0.08 \\
    SciTail & 69.35 & 70.74 & 1.39 & 71.10 & 1.75 \\
    QQP & 70.60 & 71.52 & 0.92 & 71.19 & 0.59 \\
    \midrule
    Mean & 67.97 & 68.32 & 0.34 & 68.78 & 0.81 \\
    \bottomrule
    \end{tabular}
}
\caption{The accuracy of different NLI datasets. The models are trained on SNLI ($5k$) and tested on the target datasets.
CF: Child-tuning-F. CD: Child-tuning-D.
}
\label{table:nli-snli}
\end{table}

